Differentially Private Simple Linear Regression

Economics and social science research often require analyzing datasets of sensitive personal information at fine granularity, with models fit to small subsets of the data. Unfortunately, such fine-grained analysis can easily reveal sensitive individual information. We study algorithms for simple linear regression that satisfy differential privacy, a constraint which guarantees that an algorithm's output reveals little about any individual input data record, even to an attacker with arbitrary side information about the dataset. We consider the design of differentially private algorithms for simple linear regression for small datasets, with tens to hundreds of datapoints, which is a particularly challenging regime for differential privacy. Focusing on a particular application to small-area analysis in economics research, we study the performance of a spectrum of algorithms we adapt to the setting. We identify key factors that affect their performance, showing through a range of experiments that algorithms based on robust estimators (in particular, the Theil-Sen estimator) perform well on the smallest datasets, but that other more standard algorithms do better as the dataset size increases.

==> results.tex <==
\longversion{\subsection{Results}}

\longversion{
In this section we give a brief outline of the results of the experiments on each dataset before a more in-depth discussion of these results in Section~\ref{discussion}. 

A note on the statement of privacy parameters in the experiments. We will state the privacy budget used to compute the pair $(p_{25}, p_{75})$, however we will only show empirical error bounds for $p_{25}$. The empirical error bounds for $p_{75}$ display similar phenomenon. The algorithms \texttt{NoisyStats} and \texttt{DPGradDescent} inherently release both point estimates together so the privacy loss is the same whether we release the pair $(p_{25}, P_{75})$ or just $p_{25}$. However, \texttt{DPExpTheilSen}, \texttt{DPExpWideTheilSen}, \texttt{DPSSTheilSen} and the algorithm used by the Opportunity Insights team use half their budget to release $p_{25}$ and half their budget to release $p_{75}$, separately. 
}

\longversion{
\subsubsection{Opportunity Insights Data}

We compared the differentially private algorithms with each other, as well as to the the heuristic methods used by Chetty and Friedman \cite{ChettyF19}. A summary of the performance of all the algorithms on tracts in IL and NC can be found in Figure~\ref{OIdata}.
For each algorithm and state, we build an empirical cumulative density distribution of the empirical error bounds over the tracts in that state. The vertical dotted line in Figures~\ref{fig:IL_CDF}~and~\ref{fig:NC_CDF} intercepts each curve at the point as which the \emph{noise due to privacy exceeds the standard error}.
Recall that we want $\ci/\olsstd$ to be small since this can be interpreted as saying that the additional randomness injected by the DP algorithm is dominated by the randomness that was already inherent in the data from the sampling process. In both IL and NC we find that \texttt{DPSSTheilSen} and \texttt{DPExpTheilSen} are the best performing algorithms for the majority of datasets. In particular, both \texttt{DPExpTheilSen} and \texttt{DPSSTheilSen} outperformed the heuristic algorithm used by the Opportunity Insights team on the OI data.  
For the data from IL and NC, 
\texttt{DPSSTheilSen} and \texttt{DPExpTheilSen} both produce empirical error bounds that are
within the standard error for over $70\%$ of the tracts. In addition, the empirical error bounds for \texttt{DPSSTheilSen}, \texttt{DPExpTheilSen}
and the OI algorithm are within three times the standard error for $95\%$ of the tracts. }

\longversion{
\subsubsection{Washington, DC Bikeshare UCI Dataset}

Figure~\ref{bike} compares the various DP linear regression algorithms on the Bikeshare data with $\eps=2$. The metric of performance is the same as with the experiments on OI data. As with the OI data, we see that the performance of \texttt{NoisyStats} and \texttt{DPGradDescent} are roughly the same. In this regime, we see the non-robust estimators (\texttt{NoisyStats} and \texttt{GradDescent}) are outperformed on the majority of tracts by the TheilSen based estimators. Also notice at \texttt{DPWideTheilSen} and \texttt{DPExpTheilSen} both perform well on the majority of tracts. However, there is a small subset of tracts where \texttt{DPExpTheilSen} performs poorly, while \texttt{DPWideTheilSen} continues to perform well.

\begin{figure}
\includegraphics[width=0.4\textwidth]{figures/bikeeps10.png}
\caption{Bikeshare data. Empiricial CDFs of the performance over the set of datasets when $\eps=1$. }\label{bike}
\end{figure}}

\longversion{
\subsubsection{Carbon Nanotubes UCI Dataset}

A summary of the performance of the private algorithms when $\eps=0.1$ can be found in Figure~\ref{carbon}. Note that the figure displays the empirical cumulative density function of the output distribution on a single dataset, which is different to the form of the empirical CDFs in Figures~\ref{OIdata}~and~\ref{bike}. We can see that \texttt{DPExpTheilSenMatch} is the best performing algorithm, followed by \texttt{DPSSTheilSenMatch}. The fact that \texttt{DPWideTheilSenMatch} performs poorly is unsurprising given that the widening parameter $\theta=0.01$ is much larger than the standard error. Also note that \texttt{DPExpTheilSenMatch} and \texttt{DPSSTheilSenMatch} are both biased estimators. This is a result of the fact that they are estimating the TheilSen median, not the OLS median. Both \texttt{NoisyStats} and \texttt{GradDescent} are among the worst performing private algorithms on this dataset.

In Figure~\ref{morecarbon} (found in the appendix) we see that even when $\eps=0.1$, the variance of \texttt{DPExpTheilSen} does not exceed the standard error. Additionally, when $\eps=10$, \texttt{DPSSTheilSen} performs as well as \texttt{DPExpTheilSen}.}

\longversion{
\begin{figure}
\includegraphics[width=0.4\textwidth]{figures/carboneps1}
\caption{Carbon Nanotubes Data. Empirical CDF of the output distribution of the estimate of $p_{25}$ after 100 trials of each algorithm with $\eps=1$. The grey region includes all the values that are within one standard error of $\estolsstd$. The curve labelled ``standard error`` shows the non-private posterior belief on the value of the $p_{25}$ assuming Gaussian noise.
}\label{carbon}
\end{figure}}

\longversion{
\subsubsection{Stock Exchange UCI Dataset}

A summary of the performance of the private algorithms on the Stock Exchange UCI Dataset when $\eps=1$ can be found in Figure~\ref{stock}. Again on this dataset we see that \texttt{DPExpTheilSen} is the best performing algorithm, closely followed by \texttt{DPSSTheilSen} and \texttt{DPWideTheilSen}. For all three of the TheilSen based algorithms the noise added for privacy is less than the standard error. 

\begin{figure}
\includegraphics[width=0.4\textwidth]{figures/stockeps2.png}
\caption{
Stock Exchange UCI Data. Empirical cdf of the output distribution of the estimate of $p_{25}$ after 100 trials of each algorithm with $\eps=2$. The grey region includes all the values that are within one standard error of $\estolsstd$. The curve labelled ``standard error`` shows the non-private posterior belief on the value of the $p_{25}$ assuming Gaussian noise.}\label{stock}
\end{figure}}

\longversion{
\subsubsection{Synthetic Data}

The results of the synthetic data experiments are contained in Figures~\ref{fig:synth-algs-ground-truth} and \ref{fig:synth-ns-ts-ground-truth}. Recall that in our synthetic data experiments the independent variables, $x_i, i=1, \ldots, n$, are sampled from a Gaussian distribution, and the distribution of the noise of the independent variable, $F_e$, is also Gaussian. Note that we expect $\citrue(68)/\sigma(p_{25})\approx 1$ for this type of data\footnote{The slight deviation from the horizontal line at 1 for non-private OLS in all of these plots is due to the clipping of the datapoints to be within $[0,1]\times[0,1]$.} 

 In all our experiments on this type of data, for small $\sigma_e^2$ and $\eps\nvar(\bx)>400$ \texttt{NoisyStats} is the best performing algorithm. The main reason for this appears to be that in this parameter regime, the additional noise due to privacy in \texttt{NoisyStats} is less than the difference between the non-private OLS and TheilSen point estimates. When $\eps\nvar(\bx)\le400$, \texttt{DPExpTheilSen} is either the best performing algorithm or close in accuracy to the best performing algorithm. }
